On excitable beta-skeletons

A beta-skeleton is a planar proximity undirected graph of an Euclidean point set where nodes are connected by an edge if their lune-based neighborhood contains no other points of the given set. Parameter $\beta$ determines size and shape of the nodes' neighborhoods. In an excitable beta-skeleton every node takes three states --- resting, excited and refractory, and updates its state in discrete time depending on states of its neighbors. We design families of beta-skeletons with absolute and relative thresholds of excitability and demonstrate that several distinct classes of space-time excitation dynamics can be selected using beta. The classes include spiral and target waves of excitation, branching domains of excitation and oscillating localizations.

==> figs/average.tex <==
3.971 3.649 3.477 3.295 3.157 3.023 2.905 2.799 2.703 2.607 
4.1255 3.8225 3.5775 3.362 3.201 3.053 2.946 2.8475 2.7435 2.6495 
4.2373333 3.957 3.707 3.4916666 3.319 3.179 3.0403333 2.9203334 2.8063333 2.7056668 
4.24975 3.94975 3.72225 3.51525 3.33625 3.17825 3.05375 2.94075 2.81875 2.72025 
4.3368 4.0324 3.7842 3.577 3.395 3.239 3.0994 2.975 2.8746 2.7686 
4.423 4.1281667 3.8715 3.6558332 3.4731667 3.3031666 3.1641667 3.0245 2.9111667 2.7981668 
4.481 4.1835713 3.9378572 3.7192857 3.5224285 3.345 3.1932857 3.0552857 2.9372857 2.827 
4.563125 4.255625 3.995125 3.771875 3.585375 3.421375 3.278875 3.141875 3.012875 2.898375 
4.628667 4.325778 4.067111 3.8413334 3.6458888 3.4696667 3.3176668 3.1705556 3.0381112 2.9134445 
4.6898 4.37 4.1049 3.8653 3.6645 3.4997 3.3461 3.2025 3.0683 2.9453 
4.76 4.453273 4.1825457 3.9532728 3.7383637 3.5665455 3.4050908 3.258909 3.126909 2.9973636 
4.8535833 4.539583 4.26275 4.036083 3.8229167 3.6465833 3.47575 3.3119166 3.1679168 3.02175 
4.9218464 4.6138463 4.328231 4.093154 3.883 3.6811538 3.515923 3.356846 3.2145386 3.0799232 
5.004643 4.6839285 4.408214 4.1695 3.952143 3.7538571 3.5672858 3.3950715 3.2332144 3.0985 
5.0714 4.7396665 4.4728665 4.227667 4.0078 3.8112667 3.6183333 3.4451334 3.2871332 3.1364667 


==> figs/average1.tex <==
\begin{displaymath}
\begin{array}{l|lllllllllll}
  \phi  \backslash \beta  	   
      &	1.0	&	1.1	&	1.2	&	1.3	&	1.4	&	1.5	&	1.6	&	1.7	&	1.8	&	1.9	&	2.0	\\ \hline
0.027	&	4.0	&	3.6	&	3.5	&	3.3	&	3.2	&	3.0	&	2.9	&	2.8	&	2.7	&	2.6	&	2.5	\\
0.054	&	4.1	&	3.8	&	3.6	&	3.4	&	3.2	&	3.1	&	2.9	&	2.8	&	2.7	&	2.6	&	2.6	\\
0.081	&	4.2	&	3.9	&	3.7	&	3.5	&	3.3	&	3.2	&	3.0	&	2.9	&	2.8	&	2.7	&	2.6	\\
0.108	&	4.2	&	4.0	&	3.7	&	3.5	&	3.3	&	3.2	&	3.1	&	2.9	&	2.8	&	2.7	&	2.7	\\
0.136	&	4.3	&	4.0	&	3.8	&	3.6	&	3.4	&	3.2	&	3.1	&	3.0	&	2.9	&	2.8	&	2.7	\\
0.163	&	4.4	&	4.1	&	3.9	&	3.7	&	3.5	&	3.3	&	3.2	&	3.0	&	2.9	&	2.8	&	2.7	\\
0.190	&	4.5	&	4.2	&	3.9	&	3.7	&	3.5	&	3.3	&	3.2	&	3.1	&	2.9	&	2.8	&	2.7	\\
0.217	&	4.6	&	4.3	&	4.0	&	3.8	&	3.6	&	3.4	&	3.3	&	3.1	&	3.0	&	2.9	&	2.8	\\
0.244	&	4.6	&	4.3	&	4.1	&	3.8	&	3.6	&	3.5	&	3.3	&	3.2	&	3.0	&	2.9	&	2.8	\\
0.271	&	4.7	&	4.4	&	4.1	&	3.9	&	3.7	&	3.5	&	3.3	&	3.2	&	3.1	&	2.9	&	2.8	\\
0.298	&	4.8	&	4.5	&	4.2	&	4.0	&	3.7	&	3.6	&	3.4	&	3.3	&	3.1	&	3.0	&	2.9	\\
0.325	&	4.9	&	4.5	&	4.3	&	4.0	&	3.8	&	3.6	&	3.5	&	3.3	&	3.2	&	3.0	&	2.9	\\
0.353	&	4.9	&	4.6	&	4.3	&	4.1	&	3.9	&	3.7	&	3.5	&	3.4	&	3.2	&	3.1	&	2.9	\\
0.380	&	5.0	&	4.7	&	4.4	&	4.2	&	4.0	&	3.8	&	3.6	&	3.4	&	3.2	&	3.1	&	3.0	\\
0.407	&	5.1	&	4.7	&	4.5	&	4.2	&	4.0	&	3.8	&	3.6	&	3.4	&	3.3	&	3.1	&	3.0	\\
\end{array}
\end{displaymath}

